AttEntropy: On the Generalization Ability of Supervised Semantic Segmentation Transformers to New Objects in New Domains

In addition to impressive performance, vision transformers have demonstrated remarkable abilities to encode information they were not trained to extract. For example, this information can be used to perform segmentation or single-view depth estimation even though the networks were only trained for image recognition. We show that a similar phenomenon occurs when explicitly training transformers for semantic segmentation in a supervised manner for a set of categories: Once trained, they provide valuable information even about categories absent from the training set. This information can be used to segment objects from these never-seen-before classes in domains as varied as road obstacles, aircraft parked at a terminal, lunar rocks, and maritime hazards.

==> fig/fig_quali_domain_tour.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure} [ht]
\centering

\begin{tabular}{cc}
\hspace{-3mm}\includegraphics[height=0.22\linewidth]{images/quali_domain_tour/curvy-street_carton_6_image_cut.jpg}
\hspace{-3mm}\includegraphics[height=0.22\linewidth]{images/quali_domain_tour/curvy-street_carton_6_heat_cut.jpg}
&
\hspace{-3mm}\includegraphics[height=0.22\linewidth]{images/quali_domain_tour/aircraft_image.jpg}
\hspace{-3mm}\includegraphics[height=0.22\linewidth]{images/quali_domain_tour/aircraft_heat.jpg}\\
% {\small Unusual road obstacles\\\cite{Chan21b}} & {\small Aircrafts\\ \cite{AirbusAircraftSegmentation}} \\
{\small Unusual road obstacles } & {\small Aircrafts } \\

\hspace{-3mm}\includegraphics[height=0.22\linewidth]{images/quali_domain_tour/8641_image_cut.jpg}
\hspace{-3mm}\includegraphics[height=0.22\linewidth]{images/quali_domain_tour/8641_heat_cut.jpg}
&
\hspace{-3mm}\includegraphics[height=0.22\linewidth]{images/quali_domain_tour/1032_image_cut.jpg}
\hspace{-3mm}\includegraphics[height=0.22\linewidth]{images/quali_domain_tour/1032_heat_cut.jpg}\\
Lunar rocks  & Maritime hazards 
% Lunar rocks\\\cite{ArtificialLunarLandscape} & Maritime hazards\\\cite{Bovcon19}
\end{tabular}
\vspace{-3mm}
\caption{\small {\bf Segmenting objects from categories the network was {\it not} trained for.}
The attention-entropy extracted from a SETR~\cite{\citeSETR} transformer trained on the urban driving Cityscapes~\cite{Cordts16} dataset lets us segment objects from four previously unseen categories In all four cases, we show an original image and the corresponding Attention Entropy.}
\label{fig:qualiDomainTour}
\end{figure}


% \includegraphics[height=0.45\linewidth]{images/quali_domain_tour/air_12210ad7-83f8-4b54-bb4b-e93f8ff6ac1f_setr.jpg}

% \includegraphics[height=0.45\linewidth]{images/quali_domain_tour/curvy-street_carton_6_setr.jpg}
% \includegraphics[height=0.45\linewidth]{images/quali_domain_tour/maritime_1032_img_and_setr.jpg}
% \includegraphics[height=0.45\linewidth]{images/quali_domain_tour/air_12210ad7-83f8-4b54-bb4b-e93f8ff6ac1f_setr.jpg}

==> fig/fig_quali_lunar.tex <==

\begin{figure} 
\centering
%
{\tiny
\includegraphics[width=0.30\linewidth]{images/quali_lunar/0011_img.jpg}
\includegraphics[width=0.30\linewidth]{images/quali_lunar/0011_setr.jpg}
\includegraphics[width=0.30\linewidth]{images/quali_lunar/0011_segf.jpg}
\makebox[0.3\linewidth]{\small Input} \makebox[0.3\linewidth]{\small Ours SETR}\makebox[0.3\linewidth]{\small Ours Segformer}

\includegraphics[width=0.30\linewidth]{images/quali_lunar/0011_odin.jpg}
\includegraphics[width=0.30\linewidth]{images/quali_lunar/0011_maxsoftmax.jpg}
\makebox[0.49\linewidth]{\small ODIN} \makebox[0.49\linewidth]{\small Max Softmax}

\includegraphics[width=0.30\linewidth]{images/quali_lunar/0011_lost.jpg}
\includegraphics[width=0.30\linewidth]{images/quali_lunar/0011_dino.jpg}
\includegraphics[width=0.30\linewidth]{images/quali_lunar/0011_synboost.jpg}
\makebox[0.3\linewidth]{\small LOST} \makebox[0.3\linewidth]{\small DINO}\makebox[0.3\linewidth]{\small SynBoost}
}
%
\caption{Qualitative results on obstacle detection on Lunar dataset~\cite{ArtificialLunarLandscape}.
The contour of the ground truth obstacle areas is highlighted.
%Compared to the other training-free obstacle detection methods, our attention entropy generalizes better to the distant domain of maritime scenes.
}
\label{fig:sup_quali_lunar}
\end{figure}


==> fig/fig_quali_weather_h.tex <==

\begin{figure*} 
\centering
%
\includegraphics[width=0.49\linewidth]{images/quali_segme/horiz/snowstorm2_00_00_52.502_q.jpg}
\includegraphics[width=0.49\linewidth]{images/quali_segme/horiz/driveway_bagO_ball_3_q.jpg}
% \includegraphics[width=0.2\linewidth]{images/quali_water/0041.jpg}
% \includegraphics[width=0.19\linewidth]{images/quali_water/0200.jpg}
%
\caption{Qualitative results on RoadObstacle21~\cite{Chan21b} dataset with difficult weather and limited light.
The middle and right columns show the averaged entropy of SETR and Segformer respectively, both using manual layer averaging.
Slight rectangular artifacts arise from MMSegmentation's sliding window inference.
}
\label{fig:quali_weather}
\end{figure*}


==> fig/fig_sup_quali_water.tex <==

\begin{figure} 
\centering
%
\includegraphics[width=0.30\linewidth]{images/sup_quali_water/0361_img.jpg}
\includegraphics[width=0.30\linewidth]{images/sup_quali_water/0361_ours.jpg}
\includegraphics[width=0.30\linewidth]{images/sup_quali_water/0361_segf.jpg}
\makebox[0.3\linewidth]{\small Input} \makebox[0.3\linewidth]{\small Ours SETR}\makebox[0.3\linewidth]{\small Ours Segformer}

\includegraphics[width=0.30\linewidth]{images/sup_quali_water/0361_mahalanobis.jpg}
\includegraphics[width=0.30\linewidth]{images/sup_quali_water/0361_odin.jpg}
\includegraphics[width=0.30\linewidth]{images/sup_quali_water/0361_maxsoft.jpg}
\makebox[0.3\linewidth]{\small Mahalanobis} \makebox[0.3\linewidth]{\small ODIN}\makebox[0.3\linewidth]{\small Max Softmax}

\includegraphics[width=0.30\linewidth]{images/sup_quali_water/0361_lost.jpg}
\includegraphics[width=0.30\linewidth]{images/sup_quali_water/0361_dino.jpg}
\includegraphics[width=0.30\linewidth]{images/sup_quali_water/0361_synboost.jpg}
\makebox[0.3\linewidth]{\small LOST} \makebox[0.3\linewidth]{\small DINO}\makebox[0.3\linewidth]{\small SynBoost}
%
\caption{Qualitative results on obstacle detection on Maritime Dataset ~\cite{Bovcon19}.
The contour of the ground truth obstacle areas is highlighted.
Compared to the other training-free obstacle detection methods, our attention entropy generalizes better to the distant domain of maritime scenes.
 }
\label{fig:sup_quali_water}
\end{figure}


==> fig/table_lunar.tex <==

\begin{table}[t]
\centering
\setlength{\heavyrulewidth}{2pt}
% \setlength{\arrayrulewidth}{1pt}
{ \tiny
\begin{tabular}{l|rrrrr}
\toprule
% {} & AP $\uparrow$ & FPR$_{95}$ $\downarrow$ \\
{} & AP $\uparrow$ & FPR$_{95}$ $\downarrow$ & $\overline{\mbox{sIoU}}\uparrow$ & $\overline{\mbox{PPV}}\uparrow$ & $\overline{F_1}\uparrow$ \\
\midrule
Ours SETR & 34.7 & 87.6 & {\bf 7.0} & 26.6 & {\bf 6.9} \\
Ours DPT & 35.1 & 89.9 & 4.0 & 37.7 & 5.1 \\
Ours Segformer & 34.0 & 87.5 & 5.0 & 34.1 & 4.3 \\
% Maximized Entropy \cite{Chan21a} & 41.5 & 81.0 & 5.0 & 43.5 & 6.0 \\
% Ours Segformer$_{manual}$ & {\bf 37.8} & 76.1 & 5.6 & 38.2 & 5.1 \\
% LOST-vit_small16_k__invDeg & 37.0 & 92.7 & 5.6 & 31.9 & 5.1 \\
% Ours SETR & 35.9 & 85.0 & 7.9 & 29.8 & {\bf 8.3} \\
SynBoost \cite{DiBlase21} & {\bf 35.6} & 81.9 & 4.0 & 28.8 & 3.6 \\
DINO \cite{caron2021emerging} & 32.5 & 93.0 & 6.1 & 22.4 & 4.3 \\
ODIN \cite{Liang18b} & 29.7 & {\bf 75.1} & 2.6 & 33.6 & 2.3 \\
% Max Softmax \cite{Hendrycks17b} & 28.5 & 75.1 & 2.2 & 33.2 & 1.9 \\
Max Softmax & 28.5 & {\bf 75.1} & 2.2 & 33.2 & 1.9 \\
LOST \cite{LOST} & 18.4 & 94.9 & 0.6 & {\bf 39.4} & 0.5 \\
\bottomrule
\end{tabular}
}	
\vspace{1pt}
\caption{\textbf{Obstacle pixel segmentation performance in the Artificial Lunar Landscape~\cite{ArtificialLunarLandscape} dataset}.
The evaluation was performed on every 10-th image due to big dataset size.
The primary metrics are Average Precision (AP$\uparrow$) for pixel classification and Average $F_1$ ($\overline{F_1}\uparrow$) for instance level detection.
}
\label{table:lunar}
\end{table}


==> fig/table_lunar_maritime.tex <==
\begin{table}[tb]
\parbox[b]{.53\linewidth}{
    \centering
    \setlength{\heavyrulewidth}{1pt}
    % \setlength{\arrayrulewidth}{1pt}
    \resizebox{0.95\linewidth}{!}{
    {
    \begin{tabular}{l|rrrrr}
    \toprule
    % {} & AP $\uparrow$ & FPR$_{95}$ $\downarrow$ \\
    {} & AP $\uparrow$ & FPR$_{95}$ $\downarrow$ & $\overline{\mbox{sIoU}}\uparrow$ & $\overline{\mbox{PPV}}\uparrow$ & $\overline{F_1}\uparrow$ \\
    \midrule
    Ours SETR & 34.7 & 87.6 & {\bf 7.0} & 26.6 & {\bf 6.9} \\
    Ours DPT & 35.1 & 89.9 & 4.0 & 37.7 & 5.1 \\
    Ours Segformer & 34.0 & 87.5 & 5.0 & 34.1 & 4.3 \\
    % Maximized Entropy \cite{Chan21a} & 41.5 & 81.0 & 5.0 & 43.5 & 6.0 \\
    % Ours Segformer$_{manual}$ & {\bf 37.8} & 76.1 & 5.6 & 38.2 & 5.1 \\
    % LOST-vit_small16_k__invDeg & 37.0 & 92.7 & 5.6 & 31.9 & 5.1 \\
    % Ours SETR & 35.9 & 85.0 & 7.9 & 29.8 & {\bf 8.3} \\
    SynBoost \cite{DiBlase21} & {\bf 35.6} & 81.9 & 4.0 & 28.8 & 3.6 \\
    DINO \cite{caron2021emerging} & 32.5 & 93.0 & 6.1 & 22.4 & 4.3 \\
    ODIN \cite{Liang18b} & 29.7 & {\bf 75.1} & 2.6 & 33.6 & 2.3 \\
    % Max Softmax \cite{Hendrycks17b} & 28.5 & 75.1 & 2.2 & 33.2 & 1.9 \\
    Max Softmax & 28.5 & {\bf 75.1} & 2.2 & 33.2 & 1.9 \\
    LOST \cite{LOST} & 18.4 & 94.9 & 0.6 & {\bf 39.4} & 0.5 \\
    \bottomrule
    \end{tabular}
    }	} \vspace{10pt}
    \caption{\textbf{Obstacle pixel segmentation performance in the Lunar~\cite{ArtificialLunarLandscape} dataset}.
    The evaluation was performed on every 10-th image due to the big dataset size.
    The primary metrics are Average Precision (AP$\uparrow$) for pixel classification and Average $F_1$ ($\overline{F_1}\uparrow$) for instance level detection.
    }%
    \label{table:lunar}%
}\hfill
\parbox[b]{.43\linewidth}{
    \centering
    \setlength{\heavyrulewidth}{1pt}
    % \setlength{\arrayrulewidth}{1pt}
    \resizebox{0.75\linewidth}{!}{
    \begin{tabular}{l|rr}
    \toprule
    {} & AP $\uparrow$ & FPR$_{95}$ $\downarrow$ \\
    \midrule
    Ours SETR  & 59.6 & 39.6 \\
    Ours DPT &  \textbf{71.9} &       \textbf{14.2} \\
    % Ours SETR$_{manual}$ & \textbf{63.9} & \textbf{35.0} \\
    % LOST-vit\_small16\_k\_\_invDeg & 61.7 & 56.4 \\
    Ours Segformer & 55.8 &      51.0 \\
    % Maximized Entropy \cite{Chan21a} & 42.2 & 64.7 \\
    DINO \cite{caron2021emerging} & 41.4 & 39.5 \\
    Max Softmax  & 18.6 & 64.9 \\
    ODIN \cite{Liang18b} & 16.6 & 70.8 \\
    SynBoost \cite{DiBlase21} & 14.9 & 80.0 \\
    LOST \cite{LOST} & 10.1 & 94.4 \\
    Mahalanobis \cite{Lee18a} & 5.9 & 97.3 \\
    \bottomrule
    \end{tabular}
    }	
    \vspace{8pt}
    \caption{\textbf{Obstacle pixel segmentation performance in the Maritime dataset MaSTr1325~\cite{Bovcon19}}.
    We do not measure object-level metrics since the maritime scenes contain non-instance obstacles, such as land.
    }
    \label{table:maritime}
    }
\end{table}

==> fig/table_lunar_wrap.tex <==
\begin{wraptable}{r}{7.2cm}
    \centering
    \setlength{\heavyrulewidth}{1pt}
    % \setlength{\arrayrulewidth}{1pt}
    {\scriptsize 
    \begin{tabular}{l|rrrrr}
    \toprule
    % {} & AP $\uparrow$ & FPR$_{95}$ $\downarrow$ \\
    {} & AP $\uparrow$ & FPR$_{95}$ $\downarrow$ & $\overline{\mbox{sIoU}}\uparrow$ & $\overline{\mbox{PPV}}\uparrow$ & $\overline{F_1}\uparrow$ \\
    \midrule
    Ours SETR & 34.7 & 87.6 & {\bf 7.0} & 26.6 & {\bf 6.9} \\
    Ours DPT & 35.1 & 89.9 & 4.0 & 37.7 & 5.1 \\
    Ours Segformer & 34.0 & 87.5 & 5.0 & 34.1 & 4.3 \\
    % Maximized Entropy \cite{Chan21a} & 41.5 & 81.0 & 5.0 & 43.5 & 6.0 \\
    % Ours Segformer$_{manual}$ & {\bf 37.8} & 76.1 & 5.6 & 38.2 & 5.1 \\
    % LOST-vit_small16_k__invDeg & 37.0 & 92.7 & 5.6 & 31.9 & 5.1 \\
    % Ours SETR & 35.9 & 85.0 & 7.9 & 29.8 & {\bf 8.3} \\
    SynBoost \cite{DiBlase21} & {\bf 35.6} & 81.9 & 4.0 & 28.8 & 3.6 \\
    DINO \cite{caron2021emerging} & 32.5 & 93.0 & 6.1 & 22.4 & 4.3 \\
    ODIN \cite{Liang18b} & 29.7 & {\bf 75.1} & 2.6 & 33.6 & 2.3 \\
    % Max Softmax \cite{Hendrycks17b} & 28.5 & 75.1 & 2.2 & 33.2 & 1.9 \\
    Max Softmax & 28.5 & {\bf 75.1} & 2.2 & 33.2 & 1.9 \\
    LOST \cite{LOST} & 18.4 & 94.9 & 0.6 & {\bf 39.4} & 0.5 \\
    \bottomrule
    \end{tabular}
    }	
    \caption{\textbf{Obstacle pixel segmentation performance in the Artificial Lunar Landscape~\cite{ArtificialLunarLandscape} dataset}.
    The evaluation was performed on every 10-th image due to big dataset size.
    The primary metrics are Average Precision (AP$\uparrow$) for pixel classification and Average $F_1$ ($\overline{F_1}\uparrow$) for instance level detection.
    }%
    \label{table:lunar}%
\end{wraptable}

==> fig/table_maritime.tex <==

\begin{table}[t]
\centering
\setlength{\heavyrulewidth}{1pt}
% \setlength{\arrayrulewidth}{1pt}
{ \tiny
\begin{tabular}{l|rr}
\toprule
{} & AP $\uparrow$ & FPR$_{95}$ $\downarrow$ \\
\midrule
Ours SETR  & 59.6 & 39.6 \\
Ours DPT &  \textbf{71.9} &       \textbf{14.2} \\
% Ours SETR$_{manual}$ & \textbf{63.9} & \textbf{35.0} \\
% LOST-vit\_small16\_k\_\_invDeg & 61.7 & 56.4 \\
Ours Segformer & 55.8 &      51.0 \\
% Maximized Entropy \cite{Chan21a} & 42.2 & 64.7 \\
DINO \cite{caron2021emerging} & 41.4 & 39.5 \\
Max Softmax  & 18.6 & 64.9 \\
ODIN \cite{Liang18b} & 16.6 & 70.8 \\
SynBoost \cite{DiBlase21} & 14.9 & 80.0 \\
LOST \cite{LOST} & 10.1 & 94.4 \\
Mahalanobis \cite{Lee18a} & 5.9 & 97.3 \\
\bottomrule
\end{tabular}
}	
\vspace{1pt}
\caption{\textbf{Obstacle pixel segmentation performance in the MaSTr1325~\cite{Bovcon19} dataset}.
We do not measure object-level metrics since the maritime scenes contain non-instance obstacles, such as land.
}
\label{table:maritime}
\end{table}


==> fig/table_maritime_wrap.tex <==
\begin{wraptable}{r}{4.5cm}
    \centering
    \setlength{\heavyrulewidth}{1pt}
    % \setlength{\arrayrulewidth}{1pt}
    { \scriptsize
    \begin{tabular}{l|rr}
    \toprule
    {} & AP $\uparrow$ & FPR$_{95}$ $\downarrow$ \\
    \midrule
    Ours SETR  & 59.6 & 39.6 \\
    Ours DPT &  \textbf{71.9} &       \textbf{14.2} \\
    % Ours SETR$_{manual}$ & \textbf{63.9} & \textbf{35.0} \\
    % LOST-vit\_small16\_k\_\_invDeg & 61.7 & 56.4 \\
    Ours Segformer & 55.8 &      51.0 \\
    % Maximized Entropy \cite{Chan21a} & 42.2 & 64.7 \\
    DINO \cite{caron2021emerging} & 41.4 & 39.5 \\
    Max Softmax  & 18.6 & 64.9 \\
    ODIN \cite{Liang18b} & 16.6 & 70.8 \\
    SynBoost \cite{DiBlase21} & 14.9 & 80.0 \\
    LOST \cite{LOST} & 10.1 & 94.4 \\
    Mahalanobis \cite{Lee18a} & 5.9 & 97.3 \\
    \bottomrule
    \end{tabular}
    }	
    \vspace{8pt}
    \caption{\textbf{Obstacle pixel segmentation performance in the MaSTr1325~\cite{Bovcon19} dataset}.
    We do not measure object-level metrics since the maritime scenes contain non-instance obstacles, such as land.
    }
    \label{table:maritime}
\end{wraptable}
